Optimized Excitation Signal Design Employing Receding Horizon Control

A novel excitation signal design strategy based on a receding horizon control inspired optimization is presented. The proposed method is shown to effectively generate space-filling designs within the input space of a nonlinear dynamic process, thereby enabling sophisticated acquisition of information in previously unexplored operational areas. Additionally, the strategy can intensify the exploitation of specific operational areas during information gathering, offering flexibility in meeting application-specific requirements.

==> Signal1.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.7\textwidth,
height=0.266\textwidth,
at={(0\textwidth,0\textwidth)},
scale only axis,
xmin=1,
xmax=300,
xtick={  1, 300},
xlabel style={font=\color{white!15!black}},
xlabel={$ k $},
ymin=-0.0500000000000002,
ymax=1.05,
ytick={0, 1},
ylabel style={font=\color{white!15!black}},
ylabel={$ u(k) $},
axis background/.style={fill=white}
]
\addplot [color=mycolor1, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	0.84753302002128\\
2	0.774108126280335\\
3	0.512835665990292\\
4	0.920092644305418\\
5	0.973521652336931\\
6	0.997344648996984\\
7	0.948856689618952\\
8	0.877388986731498\\
9	0.465379507598191\\
10	0.999578232548274\\
11	0.80772730506325\\
12	0.672271236270916\\
13	0.317945633737421\\
14	0.405234473443722\\
15	0.0775368792634932\\
16	0.29049289058681\\
17	0.450262098293624\\
18	0.641635752615804\\
19	0.0580101248384485\\
20	0.014879743202217\\
21	0.777836407644681\\
22	0.0806949703460402\\
23	0.459568183534191\\
24	0.233390353362747\\
25	0.585823008936857\\
26	0.381129256476499\\
27	0.048362748334325\\
28	0.125088091634333\\
29	0.00176374666575827\\
30	0.10800728665647\\
31	0.0147496055618425\\
32	0.734913885593716\\
33	0.120898822249425\\
34	0.844652417787778\\
35	0.0109136582786321\\
36	0.311783822255857\\
37	0.0779586872623977\\
38	0.0226501745324161\\
39	0.0324137500150479\\
40	0.0209558079264392\\
41	0.254804561635439\\
42	0.464949552917617\\
43	0.0936232684446952\\
44	0.0121840748635759\\
45	0.0115484878107823\\
46	0.00104012293665232\\
47	0.120840168738917\\
48	0.0768181157303677\\
49	0.84509705829484\\
50	0.998364417584509\\
51	0.076026425013269\\
52	0.131404694867836\\
53	0.926056475966591\\
54	0.997318319898327\\
55	0.00135377336863903\\
56	0.850427373009692\\
57	0.384476161172568\\
58	0.237167143894119\\
59	0.953203911554916\\
60	0.908661064260183\\
61	0.603857395781276\\
62	0.983642658030567\\
63	0.220771649314466\\
64	0.871760240875667\\
65	0.889378230326428\\
66	0.998406387579339\\
67	0.868668527842796\\
68	0.998173337883924\\
69	0.971755737280035\\
70	0.984854380337056\\
71	0.496352457065675\\
72	0.940795844418066\\
73	0.995555116625131\\
74	0.964853652247072\\
75	0.922372300436701\\
76	0.911857105182554\\
77	0.978626466240303\\
78	0.748594007815326\\
79	0.277704151668036\\
80	0.979639906126266\\
81	0.81229456008682\\
82	0.961334165143313\\
83	0.986964278834176\\
84	0.100084462561665\\
85	0.0412854198696757\\
86	0.236128147726569\\
87	0.157553145433666\\
88	0.95235437228328\\
89	0.349178190688306\\
90	0.865683292569215\\
91	0.979669977193826\\
92	0.806232034690704\\
93	0.66595260554017\\
94	0.918534797414739\\
95	0.553564241592693\\
96	0.530229891440538\\
97	0.000371898993654059\\
98	3.21988334777437e-06\\
99	0.116442989333856\\
100	0.0048200989738783\\
101	0.0337581857334267\\
102	0.502072224620797\\
103	0.0176715348203545\\
104	0.173049655057727\\
105	0.0401957522833146\\
106	0.00319749199875927\\
107	0.0338131960341934\\
108	0.131056512665256\\
109	0.0124619045989852\\
110	0.00366966456922886\\
111	0.0245537305617992\\
112	0.323174306253384\\
113	0.625483161402383\\
114	0.117008710699435\\
115	0.254064146023268\\
116	0.000175748132916712\\
117	0.0179178476276601\\
118	0.93408165732071\\
119	0.0994125662813951\\
120	0.383004393636965\\
121	0.537507347892412\\
122	0.0519972503413716\\
123	0.724049294629828\\
124	0.677909672869974\\
125	0.339354970522783\\
126	0.289393108722795\\
127	0.00429358400350555\\
128	0.565209309275666\\
129	0.198590742916141\\
130	0.964913290566498\\
131	0.892836137136875\\
132	0.611029305332581\\
133	0.635929342243944\\
134	0.947556725674647\\
135	0.32456995519486\\
136	0.769100774370153\\
137	0.928333941801439\\
138	0.72591057376925\\
139	0.827373597360159\\
140	0.990714120648303\\
141	0.97996452308025\\
142	0.889739266314136\\
143	0.57427840187608\\
144	0.994263543638893\\
145	0.934253474687603\\
146	0.999655292605298\\
147	0.947754590375065\\
148	0.993614504056475\\
149	0.604410183628044\\
150	0.935936918345616\\
151	0.999268530448682\\
152	0.856151001032855\\
153	0.990700544290899\\
154	0.991437818755819\\
155	0.854954671750755\\
156	0.379251282367176\\
157	0.145480935009027\\
158	0.0942913078514214\\
159	0.42343275864116\\
160	0.541493643926395\\
161	0.679656451473398\\
162	0.0709454521079689\\
163	0.619887937918758\\
164	0.06255799049999\\
165	0.00708964486902484\\
166	0.227078443435773\\
167	0.421068221707788\\
168	0.362423208535435\\
169	0.07213112087233\\
170	0.329994099095631\\
171	0.245729041934483\\
172	0.0100550433051156\\
173	0.205062965442086\\
174	0.0460443524267287\\
175	0.0403341861740915\\
176	0.0264434708779604\\
177	0.0139557280298884\\
178	0.0243768653965575\\
179	0.000244634158004781\\
180	0.0671585078712985\\
181	0.16792055760806\\
182	0.484187890991853\\
183	0.352998185457123\\
184	0.585204840272207\\
185	0.424091107790554\\
186	0.626970761751512\\
187	0.334928268272438\\
188	0.242271088106561\\
189	0.88164681101504\\
190	0.590288347113181\\
191	0.453920940287092\\
192	0.802462439249107\\
193	0.0953595271688408\\
194	0.711932976387064\\
195	0.527551950879968\\
196	0.98400113224033\\
197	0.715502117397136\\
198	0.127499422282006\\
199	0.21738330797481\\
200	0.580132753946115\\
201	0.875120652151939\\
202	0.965159165037963\\
203	0.989679952661766\\
204	0.859681300794796\\
205	0.983649015723042\\
206	0.971126380260477\\
207	0.968743275911193\\
208	0.543217078718091\\
209	0.999273281598232\\
210	0.999248366283143\\
211	0.955054120075244\\
212	0.975428954472252\\
213	0.945190157376412\\
214	0.989029454996758\\
215	0.988924982085066\\
216	0.999202679175258\\
217	0.991781369895422\\
218	0.953663570981209\\
219	0.98826709061065\\
220	0.874835851177784\\
221	0.0745776790583117\\
222	0.776529890201081\\
223	0.740140466579887\\
224	0.214431511108238\\
225	0.975057729429752\\
226	0.654047736279507\\
227	0.975720309045756\\
228	0.999887877445704\\
229	9.46645913296435e-05\\
230	0.144983078395079\\
231	0.716819779200872\\
232	0.408381268980667\\
233	0.452574292491237\\
234	0.56986886178346\\
235	0.0143840571181971\\
236	0.992265389327688\\
237	0.271656824521082\\
238	0.68772656842657\\
239	0.816553788974722\\
240	0.0050428436931337\\
241	0.148133177925697\\
242	0.225842470344824\\
243	0.522968277202156\\
244	0.0321012202432489\\
245	0.000190523079676551\\
246	0.9700066952989\\
247	0.00113844713779924\\
248	0.0200567047189842\\
249	0.761037570515346\\
250	0.00938707759364209\\
251	2.16259917173301e-05\\
252	0.000449550547414724\\
253	0.00329946816905605\\
254	0.0794930889563456\\
255	0.125635508851038\\
256	0.0787193887900299\\
257	0.00305092987759076\\
258	2.54164119328652e-05\\
259	0.0042026509497173\\
260	0.00163190077315238\\
261	0.102053991040056\\
262	5.86312259890755e-05\\
263	0.642841620179646\\
264	0.0450306620713772\\
265	0.0280763726214993\\
266	0.0226088130449212\\
267	0.980685331351834\\
268	0.622297720387876\\
269	0.63667102969491\\
270	0.653842381101143\\
271	0.652527352433756\\
272	0.506944805441244\\
273	0.987148874093399\\
274	0.898932715435489\\
275	0.434388409806052\\
276	0.229234909519935\\
277	0.934173250028375\\
278	0.980287971601202\\
279	0.47473843773028\\
280	0.971002190702632\\
281	0.706277971698493\\
282	0.480780980722622\\
283	0.940704313798526\\
284	0.58521347794172\\
285	0.93792025839565\\
286	0.376196603051605\\
287	0.980327726559478\\
288	0.184576896906427\\
289	0.00178086852072985\\
290	0.74283166946886\\
291	0.0226427791573129\\
292	0.30874935902801\\
293	0.397280222460524\\
294	0.544702673015226\\
295	0.0988418865412038\\
296	0.993069059791668\\
297	0.899818944790286\\
298	0.627379104814333\\
299	0.977916235399773\\
300	0.194730115204145\\
};
\end{axis}
\end{tikzpicture}%
